Greedy Decentralized Auction-based Task Allocation for Multi-Agent Systems

We propose a decentralized auction-based algorithm for the solution of dynamic task allocation problems for spatially distributed multi-agent systems. In our approach, each member of the multi-agent team is assigned to at most one task from a set of spatially distributed tasks, while several agents can be allocated to the same task. The task assignment is dynamic since it is updated at discrete time stages (iterations) to account for the current states of the agents as the latter move towards the tasks assigned to them at the previous stage. Our proposed methods can find applications in problems of resource allocation by intelligent machines such as the delivery of packages by a fleet of unmanned or semi-autonomous aerial vehicles. In our approach, the task allocation accounts for both the cost incurred by the agents for the completion of their assigned tasks (e.g., energy or fuel consumption) and the rewards earned for their completion (which may reflect, for instance, the agents' satisfaction). We propose a Greedy Coalition Auction Algorithm (GCAA) in which the agents possess bid vectors representing their best evaluations of the task utilities. The agents propose bids, deduce an allocation based on their bid vectors and update them after each iteration. The solution estimate of the proposed task allocation algorithm converges after a finite number of iterations which cannot exceed the number of agents. Finally, we use numerical simulations to illustrate the effectiveness of the proposed task allocation algorithm (in terms of performance and computation time) in several scenarios involving multiple agents and tasks distributed over a spatial 2D domain.

==> Figures/RewardSuccessProbabilityUtility.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}[scale=0.6]

\begin{axis}[%
width=4.521in,
height=3.461in,
at={(0.758in,0.586in)},
scale only axis,
xmin=0,
xmax=1,
tick align=outside,
xlabel style={font=\color{white!15!black}},
xlabel={Nominal reward},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={Task success probability},
zmin=0,
zmax=50,
view={-37.5}{30},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
axis z line*=left,
xmajorgrids,
ymajorgrids,
zmajorgrids
]

\addplot3[%
surf,
shader=flat corner, draw=black, z buffer=sort, colormap={mymap}{[1pt] rgb(0pt)=(0.2422,0.1504,0.6603); rgb(1pt)=(0.25039,0.164995,0.707614); rgb(2pt)=(0.257771,0.181781,0.751138); rgb(3pt)=(0.264729,0.197757,0.795214); rgb(4pt)=(0.270648,0.214676,0.836371); rgb(5pt)=(0.275114,0.234238,0.870986); rgb(6pt)=(0.2783,0.255871,0.899071); rgb(7pt)=(0.280333,0.278233,0.9221); rgb(8pt)=(0.281338,0.300595,0.941376); rgb(9pt)=(0.281014,0.322757,0.957886); rgb(10pt)=(0.279467,0.344671,0.971676); rgb(11pt)=(0.275971,0.366681,0.982905); rgb(12pt)=(0.269914,0.3892,0.9906); rgb(13pt)=(0.260243,0.412329,0.995157); rgb(14pt)=(0.244033,0.435833,0.998833); rgb(15pt)=(0.220643,0.460257,0.997286); rgb(16pt)=(0.196333,0.484719,0.989152); rgb(17pt)=(0.183405,0.507371,0.979795); rgb(18pt)=(0.178643,0.528857,0.968157); rgb(19pt)=(0.176438,0.549905,0.952019); rgb(20pt)=(0.168743,0.570262,0.935871); rgb(21pt)=(0.154,0.5902,0.9218); rgb(22pt)=(0.146029,0.609119,0.907857); rgb(23pt)=(0.138024,0.627629,0.89729); rgb(24pt)=(0.124814,0.645929,0.888343); rgb(25pt)=(0.111252,0.6635,0.876314); rgb(26pt)=(0.0952095,0.679829,0.859781); rgb(27pt)=(0.0688714,0.694771,0.839357); rgb(28pt)=(0.0296667,0.708167,0.816333); rgb(29pt)=(0.00357143,0.720267,0.7917); rgb(30pt)=(0.00665714,0.731214,0.766014); rgb(31pt)=(0.0433286,0.741095,0.73941); rgb(32pt)=(0.0963952,0.75,0.712038); rgb(33pt)=(0.140771,0.7584,0.684157); rgb(34pt)=(0.1717,0.766962,0.655443); rgb(35pt)=(0.193767,0.775767,0.6251); rgb(36pt)=(0.216086,0.7843,0.5923); rgb(37pt)=(0.246957,0.791795,0.556743); rgb(38pt)=(0.290614,0.79729,0.518829); rgb(39pt)=(0.340643,0.8008,0.478857); rgb(40pt)=(0.3909,0.802871,0.435448); rgb(41pt)=(0.445629,0.802419,0.390919); rgb(42pt)=(0.5044,0.7993,0.348); rgb(43pt)=(0.561562,0.794233,0.304481); rgb(44pt)=(0.617395,0.787619,0.261238); rgb(45pt)=(0.671986,0.779271,0.2227); rgb(46pt)=(0.7242,0.769843,0.191029); rgb(47pt)=(0.773833,0.759805,0.16461); rgb(48pt)=(0.820314,0.749814,0.153529); rgb(49pt)=(0.863433,0.7406,0.159633); rgb(50pt)=(0.903543,0.733029,0.177414); rgb(51pt)=(0.939257,0.728786,0.209957); rgb(52pt)=(0.972757,0.729771,0.239443); rgb(53pt)=(0.995648,0.743371,0.237148); rgb(54pt)=(0.996986,0.765857,0.219943); rgb(55pt)=(0.995205,0.789252,0.202762); rgb(56pt)=(0.9892,0.813567,0.188533); rgb(57pt)=(0.978629,0.838629,0.176557); rgb(58pt)=(0.967648,0.8639,0.16429); rgb(59pt)=(0.96101,0.889019,0.153676); rgb(60pt)=(0.959671,0.913457,0.142257); rgb(61pt)=(0.962795,0.937338,0.12651); rgb(62pt)=(0.969114,0.960629,0.106362); rgb(63pt)=(0.9769,0.9839,0.0805)}, mesh/rows=11]
table[row sep=crcr, point meta=\thisrow{c}] {%
%
x	y	z	c\\
0	0	0	0\\
0	0.1	0	0\\
0	0.2	0	0\\
0	0.3	0	0\\
0	0.4	0	0\\
0	0.5	0	0\\
0	0.6	0	0\\
0	0.7	0	0\\
0	0.8	0	0\\
0	0.9	0	0\\
0	1	0	0\\
0.1	0	0	0\\
0.1	0.1	0.490281064485351	0.490281064485351\\
0.1	0.2	0.986382805086652	0.986382805086652\\
0.1	0.3	1.48425168151501	1.48425168151501\\
0.1	0.4	1.98375863974928	1.98375863974928\\
0.1	0.5	2.48375863974928	2.48375863974928\\
0.1	0.6	2.98375863974928	2.98375863974928\\
0.1	0.7	3.48375863974928	3.48375863974928\\
0.1	0.8	3.98375863974928	3.98375863974928\\
0.1	0.9	4.48375863974928	4.48375863974928\\
0.1	1	4.98375863974928	4.98375863974928\\
0.2	0	0	0\\
0.2	0.1	0.983758639749278	0.983758639749278\\
0.2	0.2	1.98375863974928	1.98375863974928\\
0.2	0.3	2.98375863974928	2.98375863974928\\
0.2	0.4	3.98375863974928	3.98375863974928\\
0.2	0.5	4.98375863974928	4.98375863974928\\
0.2	0.6	5.98375863974928	5.98375863974928\\
0.2	0.7	6.98375863974927	6.98375863974927\\
0.2	0.8	7.98375863974928	7.98375863974928\\
0.2	0.9	8.98375863974928	8.98375863974928\\
0.2	1	9.98375863974927	9.98375863974927\\
0.3	0	0	0\\
0.3	0.1	1.48375863974928	1.48375863974928\\
0.3	0.2	2.98375863974928	2.98375863974928\\
0.3	0.3	4.48375863974928	4.48375863974928\\
0.3	0.4	5.98375863974928	5.98375863974928\\
0.3	0.5	7.48375863974928	7.48375863974928\\
0.3	0.6	8.98375863974928	8.98375863974928\\
0.3	0.7	10.4837586397493	10.4837586397493\\
0.3	0.8	11.9837586397493	11.9837586397493\\
0.3	0.9	13.4837586397493	13.4837586397493\\
0.3	1	14.9837586397493	14.9837586397493\\
0.4	0	0	0\\
0.4	0.1	1.98375863974928	1.98375863974928\\
0.4	0.2	3.98375863974928	3.98375863974928\\
0.4	0.3	5.98375863974928	5.98375863974928\\
0.4	0.4	7.98375863974928	7.98375863974928\\
0.4	0.5	9.98375863974928	9.98375863974928\\
0.4	0.6	11.9837586397493	11.9837586397493\\
0.4	0.7	13.9837586397493	13.9837586397493\\
0.4	0.8	15.9837586397493	15.9837586397493\\
0.4	0.9	17.9837586397493	17.9837586397493\\
0.4	1	19.9837586397493	19.9837586397493\\
0.5	0	0	0\\
0.5	0.1	2.48375863974928	2.48375863974928\\
0.5	0.2	4.98375863974928	4.98375863974928\\
0.5	0.3	7.48375863974928	7.48375863974928\\
0.5	0.4	9.98375863974928	9.98375863974928\\
0.5	0.5	12.4837586397493	12.4837586397493\\
0.5	0.6	14.9837586397493	14.9837586397493\\
0.5	0.7	17.4837586397493	17.4837586397493\\
0.5	0.8	19.9837586397493	19.9837586397493\\
0.5	0.9	22.4837586397493	22.4837586397493\\
0.5	1	24.9837586397493	24.9837586397493\\
0.6	0	0	0\\
0.6	0.1	2.98375863974928	2.98375863974928\\
0.6	0.2	5.98375863974928	5.98375863974928\\
0.6	0.3	8.98375863974928	8.98375863974928\\
0.6	0.4	11.9837586397493	11.9837586397493\\
0.6	0.5	14.9837586397493	14.9837586397493\\
0.6	0.6	17.9837586397493	17.9837586397493\\
0.6	0.7	20.9837586397493	20.9837586397493\\
0.6	0.8	23.9837586397493	23.9837586397493\\
0.6	0.9	26.9837586397493	26.9837586397493\\
0.6	1	29.9837586397493	29.9837586397493\\
0.7	0	0	0\\
0.7	0.1	3.48375863974928	3.48375863974928\\
0.7	0.2	6.98375863974928	6.98375863974928\\
0.7	0.3	10.4837586397493	10.4837586397493\\
0.7	0.4	13.9837586397493	13.9837586397493\\
0.7	0.5	17.4837586397493	17.4837586397493\\
0.7	0.6	20.9837586397493	20.9837586397493\\
0.7	0.7	24.4837586397493	24.4837586397493\\
0.7	0.8	27.9837586397493	27.9837586397493\\
0.7	0.9	31.4837586397493	31.4837586397493\\
0.7	1	34.9837586397493	34.9837586397493\\
0.8	0	0	0\\
0.8	0.1	3.98375863974928	3.98375863974928\\
0.8	0.2	7.98375863974928	7.98375863974928\\
0.8	0.3	11.9837586397493	11.9837586397493\\
0.8	0.4	15.9837586397493	15.9837586397493\\
0.8	0.5	19.9837586397493	19.9837586397493\\
0.8	0.6	23.9837586397493	23.9837586397493\\
0.8	0.7	27.9837586397493	27.9837586397493\\
0.8	0.8	31.9837586397493	31.9837586397493\\
0.8	0.9	35.9837586397493	35.9837586397493\\
0.8	1	39.9837586397493	39.9837586397493\\
0.9	0	0	0\\
0.9	0.1	4.48375863974928	4.48375863974928\\
0.9	0.2	8.98375863974928	8.98375863974928\\
0.9	0.3	13.4837586397493	13.4837586397493\\
0.9	0.4	17.9837586397493	17.9837586397493\\
0.9	0.5	22.4837586397493	22.4837586397493\\
0.9	0.6	26.9837586397493	26.9837586397493\\
0.9	0.7	31.4837586397493	31.4837586397493\\
0.9	0.8	35.9837586397493	35.9837586397493\\
0.9	0.9	40.4837586397493	40.4837586397493\\
0.9	1	44.9837586397493	44.9837586397493\\
1	0	0	0\\
1	0.1	4.98375863974928	4.98375863974928\\
1	0.2	9.98375863974928	9.98375863974928\\
1	0.3	14.9837586397493	14.9837586397493\\
1	0.4	19.9837586397493	19.9837586397493\\
1	0.5	24.9837586397493	24.9837586397493\\
1	0.6	29.9837586397493	29.9837586397493\\
1	0.7	34.9837586397493	34.9837586397493\\
1	0.8	39.9837586397493	39.9837586397493\\
1	0.9	44.9837586397493	44.9837586397493\\
1	1	49.9837586397493	49.9837586397493\\
};
\end{axis}
\end{tikzpicture}%
